Examem: Low-Overhead Memory Instrumentation for Intelligent Memory Systems

Memory performance is often the main bottleneck in modern computing systems. In recent years, researchers have attempted to scale the memory wall by leveraging new technology such as CXL, HBM, and in- and near-memory processing. Developers optimizing for such hardware need to understand how target applications perform to fully take advantage of these systems. Existing software and hardware performance introspection techniques are ill-suited for this purpose due to one or more of the following factors: coarse-grained measurement, inability to offer data needed to debug key issues, high runtime overhead, and hardware dependence. The heightened integration between compute and memory in many proposed systems offers an opportunity to extend compiler support for this purpose. We have developed Examem, a memory performance introspection framework based on the LLVM compiler infrastructure. Examem supports developer annotated regions in code, allowing for targeted instrumentation of kernels. Examem supports hardware performance counters when available, in addition to software instrumentation. It statically records information about the instruction mix of the code and adds dynamic instrumentation to produce estimated memory bandwidth for an instrumented region at runtime. This combined approach keeps runtime overhead low while remaining accurate, with a geomean overhead under 10% and a geomean byte accuracy of 93%. Finally, our instrumentation is performed using an LLVM IR pass, which is target agnostic, and we have applied it to four ISAs.

==> Sections/New.tex <==
New developments that need to be integrated:
\begin{enumerate}
    \item Sampling (Design) -> Added, 4.2
    \begin{itemize}
        \item Performance study with graphs where we show uninstrumented performance, performance when instrumenting each and every BB, and performance impact with some sampling rate\item
        We also need to prove that our sampling is fairly representative. Maybe show stats when instrumenting everything, then when setting an interval of 10 or 100, we should obtain around 1/10th or 1/100th of the stats 
    \end{itemize}
    %\item Is \projectName accurate under the hood? What is the accuracy of memory accesses recorded? What is the accuracy of bytes read and written?
    \item Polling/data transfer interface (Design) -> Added, 4.7
    \item Eliminate any references to the MIR pass (Design) -> Done
    \item Hardware performance counters (Design) -> Added to 4.2 with sampling
    \item Findings about stack and heap cache access rates (motivation)
\end{enumerate}

Sections that are old/of reduced importance and can be commented out or trimmed:
\begin{enumerate}
    \item 3.2 MIR Pass (Mostly done)
    %\item Is \projectName accurate under the hood? What is the accuracy of memory accesses recorded? What is the accuracy of bytes read and written?
    \item 3.7 correction heuristic (Done)
    \item 5.2 and 5.3 memory bandwidth and access accuracy -> need to combine section or do something to reduce the content 
    \item 5.5 Refresh/replace case studies, maybe find example with time series
    \item 5.6 Portability sections needs to be revamped, taking into account new AArch64 data
\end{enumerate}
